Subspace Learning and Imputation for Streaming Big Data Matrices and Tensors

Extracting latent low-dimensional structure from high-dimensional data is of paramount importance in timely inference tasks encountered with `Big Data' analytics. However, increasingly noisy, heterogeneous, and incomplete datasets as well as the need for {\em real-time} processing of streaming data pose major challenges to this end. In this context, the present paper permeates benefits from rank minimization to scalable imputation of missing data, via tracking low-dimensional subspaces and unraveling latent (possibly multi-way) structure from \emph{incomplete streaming} data. For low-rank matrix data, a subspace estimator is proposed based on an exponentially-weighted least-squares criterion regularized with the nuclear norm. After recasting the non-separable nuclear norm into a form amenable to online optimization, real-time algorithms with complementary strengths are developed and their convergence is established under simplifying technical assumptions. In a stationary setting, the asymptotic estimates obtained offer the well-documented performance guarantees of the {\em batch} nuclear-norm regularized estimator. Under the same unifying framework, a novel online (adaptive) algorithm is developed to obtain multi-way decompositions of \emph{low-rank tensors} with missing entries, and perform imputation as a byproduct. Simulated tests with both synthetic as well as real Internet and cardiac magnetic resonance imagery (MRI) data confirm the efficacy of the proposed algorithms, and their superior performance relative to state-of-the-art alternatives.

==> mydefs.tex <==
\usepackage{xspace,amsmath,epsfig,subfigure,theorem,times}
\input{mysymbol.sty}

\newtheorem{assumption}{\hspace{0pt}\bf AS\hspace{-0.15cm}}
\newtheorem{lemma}{\hspace{0pt}\bf Lemma}
\newtheorem{proposition}{\hspace{0pt}\bf Proposition}
\newtheorem{observation}{\hspace{0pt}\bf Observation}
\newtheorem{theorem}{\hspace{0pt}\bf Theorem}
\newtheorem{corollary}{\hspace{0pt}\bf Corollary}
\newtheorem{fact}{\hspace{0pt}\bf Fact}
\newtheorem{remark}{\hspace{0pt}\bf Remark}
\newtheorem{test}{\hspace{0pt}\it Test Case}
\newtheorem{definition}{\hspace{0pt}\bf Definition}

\def\proof  {\hspace{0pt}{\bf{Proof: }}}
\def\remark {\hspace{0pt}{\bf{Remark }}}

\def\brvh{\breve h}
\def \E   {{\rm E}}
\def \I   {{\bf 1}}
\def \db  { ~{\rm dB}}
\def \hq  { \hat{q} }
\def \hbq {\hat{{\bf q}}}
\def \htheta  { \hat{\theta} }
\def \hsigma  { \hat{\sigma} }
\def \btheta  { {\mbox{\boldmath $\theta$}} }
\def \bbtheta  { {\mbox{\boldmath $\theta$}} }
\def \bsigma  { {\mbox{\boldmath $\psi$}} }
\def \hbtheta { {\mbox{\boldmath $\hat{\theta}$}} }

\def \argumentone     {(\Delta_{1})}
\def \functionone     {\frac{q_1 \left(1-q_1\right) }{p_v^2\argumentone}}
\def \functiononeb    {\frac{q_1 \left(1-q_1\right) }{p_v^2\argumentone \Delta_{1}^2}}
\def \argumenttwo     {(\Delta_{2})}
\def \functiontwo     {\frac{q_2 \left(1-q_2\right) }{p_v^2\argumenttwo}}
\def \functiontwob    {\frac{q_2 \left(1-q_2\right) }{p_v^2\argumenttwo \Delta_{2}^2}}
\def \functiononetwo  {\frac {q_2 \left(1-q_1\right) }{p_v\argumentone p\argumenttwo}}
\def \functiononetwob {\frac {q_2 \left(1-q_1\right) }{p_v\argumentone p\argumenttwo \Delta_{1} \Delta_{2}} }
\def \deltak          {\frac{\tau_{k} - \theta}{\sigma}}
\def \argumentk      {(\Delta_k)}
\def \functionk      {\frac{q_k \left(1-q_k\right) }{p_v^2\argumentk}}

\def \error {e_a}
\def \Q     {F_v}
\def \bby   {{\mbox{\boldmath $\beta$}} }
\def \bbby  { \beta }
\def \calB  {{\cal B}}

